Stable and high quality electron beams from staged laser and plasma wakefield accelerators

We present experimental results on a plasma wakefield accelerator (PWFA) driven by high-current electron beams from a laser wakefield accelerator (LWFA). In this staged setup stable and high quality (low divergence and low energy spread) electron beams are generated at an optically-generated hydrodynamic shock in the PWFA. The energy stability of the beams produced by that arrangement in the PWFA stage is comparable to both single-stage laser accelerators and plasma wakefield accelerators driven by conventional accelerators. Simulations support that the intrinsic insensitivity of PWFAs to driver energy fluctuations can be exploited to overcome stability limitations of state-of-the-art laser wakefield accelerators when adding a PWFA stage. Furthermore, we demonstrate the generation of electron bunches with energy spread and divergence superior to single-stage LW-FAs, resulting in bunches with dense phase space and an angular-spectral charge density beyond the initial drive beam parameters. These results unambiguously show that staged LWFA-PWFA can help to tailor the electron-beam quality for certain applications and to reduce the influence of fluctuating laser drivers on the electron-beam stability. This encourages further development of this new class of staged wakefield acceleration as a viable scheme towards compact, high-quality electron beam sources.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

